Clustering-driven Deep Embedding with Pairwise Constraints

Recently, there has been increasing interest to leverage the competence of neural networks to analyze data. In particular, new clustering methods that employ deep embeddings have been presented. In this paper, we depart from centroid-based models and suggest a new framework, called Clustering-driven deep embedding with PAirwise Constraints (CPAC), for non-parametric clustering using a neural network. We present a clustering-driven embedding based on a Siamese network that encourages pairs of data points to output similar representations in the latent space. Our pair-based model allows augmenting the information with labeled pairs to constitute a semi-supervised framework. Our approach is based on analyzing the losses associated with each pair to refine the set of constraints. We show that clustering performance increases when using this scheme, even with a limited amount of user queries. We demonstrate how our architecture is adapted for various types of data and present the first deep framework to cluster 3D shapes.

==> tables/VGG_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|ll|ll}
\hline
Dataset       & \multicolumn{2}{l|}{FRGC} & \multicolumn{2}{l}{YTF} \\ \hline
              & ami         & nmi         & ami        & nmi        \\ \hline
kmeans        & 0.58        & 0.61        & 0.74       & 0.75       \\
RCC (kmeans)  & 0.65        & 0.67        & 0.76       & 0.77       \\
DEC           &             &             &            &            \\ \hline
Ours (kmeans) & 0.63        & 0.65        & 0.79       & 0.8       
\end{tabular}
\caption{\textbf{Results on VGG19 features}}
\label{tbl:VGG_results}
\end{table}

==> tables/semi_loss_numconn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|cc|cc|cc}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\#labeled \\ connections\end{tabular}} & \multicolumn{2}{c|}{USPS} & \multicolumn{2}{c|}{FRGC} & \multicolumn{2}{c}{CMU-PIE} \\ \cline{2-7} 
                                                                                  & NMI         & ACC        & NMI         & ACC         & NMI           & ACC          \\ \hline
0                                                                                 & 0.788       & 0.576      & 0.717       & 0.519       & 0.888         & 0.547        \\
0.1k                                                                               & 0.775       & 0.572      & 0.738       & 0.516       & 0.870          & 0.636        \\
1k                                                                              & 0.881       & 0.845      & 0.778       & 0.542       & 0.879         & 0.688        \\
5k                                                                              & 0.945       & 0.959      & 0.819       & 0.570        & 0.926         & 0.796       
\end{tabular}
\caption{Semi-supervised clustering results. Above, we report the clustering performance as the number of labeled MKNN connections increases. }% percentage of labeled connections out of $N\times N$ is smaller than 0.2\% for all of the results. }
\label{tbl:semi_supervised_results}
\end{table}

==> tables/semi_supervised_loss.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{c|cc|cc|cc}
\multirow{2}{*}{\%MKNN labeled} & \multicolumn{2}{c|}{USPS} & \multicolumn{2}{c|}{FRGC} & \multicolumn{2}{c}{CMU-PIE} \\ \cline{2-7} 
                                       & NMI         & ACC         & NMI         & ACC         & NMI          & ACC          \\ \hline
0                                      & 0.788       & 0.576       & 0.717       & 0.519       & 0.888        & 0.547        \\
1\%                                    & 0.806       & 0.654       & 0.73        & 0.532       & 0.871        & 0.641        \\
3\%                                    & 0.875       & 0.842       & 0.751       & 0.525       & 0.870         & 0.647        \\
5\%                                    & 0.887       & 0.848       & 0.737       & 0.532       & 0.880         & 0.665        \\
10\%                                   & 0.937       & 0.955       & 0.744       & 0.525       & 0.884        & 0.691        \\
20\%                                   & 0.945       & 0.959       & 0.768       & 0.538       & 0.888        & 0.728        \\
30\%                                   & 0.953       & 0.962       & 0.798       & 0.549       & 0.904        & 0.736        \\
50\%                                   & 0.958       & 0.963       & 0.800         & 0.567       & 0.936        & 0.801       
\end{tabular}
\caption{Semi-supervised clustering results. Above, we report the clustering performance as the percentage of labeled MKNN connections increases. The reported scores are all obtained on less than 0.2\% out of all the entire dataset ($N\times N$ connections). }% percentage of labeled connections out of $N\times N$ is smaller than 0.2\% for all of the results. }
\label{tbl:semi_supervised_results}
\end{table}

==> tables/unsupervised_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|cc|cc|cc|cc|cc}
           & \multicolumn{2}{c|}{USPS}                                                     & \multicolumn{2}{c|}{FRGC}                                                    & \multicolumn{2}{c|}{YTF}                                                      & \multicolumn{2}{c|}{CMU-PIE}                                                  & \multicolumn{2}{c}{REUTERS}                                                       \\ \cline{2-11} 
           & NMI                                   & ACC                                   & NMI                                   & ACC                                  & NMI                                   & ACC                                   & NMI                                   & ACC                                   & NMI                                   & ACC                                   \\ \hline
DEC        & 0.586                                 & 0.619                                 & 0.505                                 & 0.378                                & 0.446                                 & 0.371                                 & 0.924                                 & 0.801                                 & \textbf{0.721}  & {\textbf{0.570}}                                \\
JULE-SF    & 0.858                                 & 0.922                                 & 0.566                                 & 0.461                                & \textbf{0.848}                                 & \textbf{0.684}                                 & 0.984                                 & 0.980                                  & -                                     & -                                     \\
JULE-RF    & 0.913                                 & 0.950                                  & 0.574                                 & 0.461                                & \textbf{0.848}                                 & \textbf{0.684}                                 & {\textbf{1.000}}     & {\textbf{1.000}}     & -                                     & -                                     \\
DEPICT     & {\textbf{0.927}} & {\textbf{0.964}} & \textbf{0.610}                                  & \textbf{0.470}                                 & 0.802                                 & 0.621                                 & 0.974                                 & 0.883                                 & -                                     & -                                     \\
% CPAC+AGL   & 0.731                                 & 0.582                                 & 0.486                                 & 0.358                                & 0.847                                 & {\textbf{0.688}} & 0.833                                 & 0.618                                 & {\textbf{0.753}} & {\textbf{0.572}} \\
\hline
AP         & 0.536                                 & 0.038                                 & 0.585                                 & 0.196                                & 0.781                                 & 0.251                                 & 0.668                                 & 0.282                                 & 0.373                                 & 0.012                                 \\
HDB        & 0.374                                 & 0.250                                  & 0.549                                 & 0.229                                & 0.841                                 & {\textbf{0.605}} & 0.699                                 & 0.239                                 & 0.300                                   & 0.223                                 \\
RCC        & 0.778                                 & 0.595                                 & 0.683                                 & 0.495                                & 0.844                                 & 0.461                                 & 0.883                                 & 0.622                                 & 0.361                                 & 0.020                                  \\
RCC-DR     & 0.763                                 & 0.520                                  & 0.598                                 & 0.430                                 &{\textbf{0.874}} & 0.444                                 & 0.515                                 & 0.232                                 & 0.369                                 & 0.020                                  \\
CPAC  & 0.788                                 & 0.576                                 & 0.717                                 & 0.519                                & 0.869                                 & 0.542                                 & {\textbf{0.888}} & 0.547                                 & {\textbf{0.401}} & {\textbf{0.236}} \\
CPAC-VGG   & {\textbf{0.914}} & {\textbf{0.867}} & {\textbf{0.799}} & {\textbf{0.540}} & 0.860                                  & 0.542                                 & 0.849                                 & {\textbf{0.688}} & -                                     & -                                    
\end{tabular}
\caption{Clustering evaluation on parametric (top rows) and non-parametric (bottom row) techniques. For each category, we emphasize the best results in bold. As the table illustrates, our non-parametric technique (bottom two rows) yields scores which are comparable to the parametric ones.}
\label{tbl:unsupervised_results}
\end{table}

==> tables/unsupervised_results2.tex <==
\begin{table}[]
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{l|cc|cc|cc|cc|cc}
         & \multicolumn{2}{c|}{USPS}                   & \multicolumn{2}{c|}{FRGC}                   & \multicolumn{2}{c|}{YTF}                    & \multicolumn{2}{c|}{CMU-PIE}                & \multicolumn{2}{c|}{REUTERS}                \\ \cline{2-11} 
         & nmi                  & acc                  & nmi                  & acc                  & nmi                  & acc                  & nmi                  & acc                  & nmi                  & acc                  \\ \hline
DEC      & 0.586                & 0.619                & 0.505                & 0.378                & 0.446                & 0.371                & 0.924                & 0.801                & \textbf\{0.721\}     & \{\textbf\{0.570\}\} \\
JULE-SF  & 0.858                & 0.922                & 0.566                & 0.461                & \textbf\{0.848\}     & \textbf\{0.684\}     & 0.984                & 0.980                & -                    & -                    \\
JULE-RF  & 0.913                & 0.950                & 0.574                & 0.461                & \textbf\{0.848\}     & \textbf\{0.684\}     & \{\textbf\{1.000\}\} & \{\textbf\{1.000\}\} & -                    & -                    \\
DEPICT   & \{\textbf\{0.927\}\} & \{\textbf\{0.964\}\} & \textbf\{0.610\}     & \textbf\{0.470\}     & 0.802                & 0.621                & 0.974                & 0.883                & -                    & -                    \\ \hline
AP       & 0.536                & 0.038                & 0.585                & 0.196                & 0.781                & 0.251                & 0.668                & 0.282                & 0.373                & 0.012                \\
HDB      & 0.374                & 0.250                & 0.549                & 0.229                & 0.841                & \{\textbf\{0.605\}\} & 0.699                & 0.239                & 0.300                & 0.223                \\
RCC      & 0.778                & 0.595                & 0.683                & 0.495                & 0.844                & 0.461                & 0.883                & 0.622                & 0.361                & 0.020                \\
RCC-DR   & 0.763                & 0.520                & 0.598                & 0.430                & \{\textbf\{0.874\}\} & 0.444                & 0.515                & 0.232                & 0.369                & 0.020                \\
CPAC     & 0.788                & 0.576                & 0.717                & 0.519                & 0.869                & 0.542                & \{\textbf\{0.888\}\} & 0.547                & \{\textbf\{0.401\}\} & \{\textbf\{0.236\}\} \\
CPAC-VGG & \{\textbf\{0.914\}\} & \{\textbf\{0.867\}\} & \{\textbf\{0.799\}\} & \{\textbf\{0.540\}\} & 0.860                & 0.542                & 0.849                & \{\textbf\{0.688\}\} & -                    & -                   
\end{tabular}
\end{table}
